Adaptive Randomized Pivoting for Tensor Cross Approximation in the T-Product Framework

This paper studies extensions of adaptive randomized pivoting (ARP), recently introduced for matrix column subset selection, to tensors in the t-product framework. We propose two constructions. ARP-T-CUR applies matrix ARP-cross at the nonredundant Fourier frequencies and uses conjugate symmetry to preserve real-valued tensors. Assuming that the selected intersections are nonsingular almost surely, the matrix theory gives a direct expected-error bound for this Fourier-slicewise approximation. T-ARP instead selects common lateral and horizontal slices, with the same indices used at every Fourier frequency. This common-index constraint requires a new analysis. Under frequency-alignment and frequency-wise rank-growth assumptions, we prove an expected-error bound and recover the matrix ARP factor $r+1$ when the frequency-wise sampling distributions are aligned. We also derive bounds for tensor cross approximation and t-DEIM. The numerical experiments show that both proposed methods give accurate tensor approximations and perform favorably against the considered slice-selection baselines. A separate full-enumeration experiment verifies the assumptions and the expected-error bound for common-index T-ARP.

==> figures/function_tensor/relative_error_plot__old_.tex <==
\definecolor{arpTCUR}{RGB}{0,114,178}
\definecolor{tSVD}{RGB}{0,0,0}
\definecolor{tUniform}{RGB}{230,159,0}
\definecolor{tLeverage}{RGB}{0,158,115}
\definecolor{tARP}{RGB}{213,94,0}
\definecolor{tARPHouseholder}{RGB}{204,121,167}
\begin{tikzpicture}
\begin{axis}[%
width=\linewidth,
height=0.82\linewidth,
xlabel={Target rank / number of selected slices per mode \(r\)},
ylabel={Relative Error (log scale)},
ymode=log,
xtick={2,4,6,8,10,12,14,16,18,20,22},
grid=both,
legend style={font=\scriptsize, at={(0.5,-0.35)}, anchor=north, legend columns=2},
]
\addplot+[color=arpTCUR, mark=square*, solid, line width=0.9pt] coordinates {(2,8.251576334724e-03) (3,1.402991311114e-03) (4,4.015374158071e-04) (5,1.501190675533e-04) (6,9.842973434472e-05) (7,5.950687536851e-05) (8,8.208075280632e-05) (9,6.697778335710e-05) (10,6.462727775895e-05) (11,7.123581784923e-05) (12,6.978514378266e-05) (13,6.580921130840e-05) (14,6.826400257841e-05) (15,7.106186389214e-05) (16,6.947022915571e-05) (17,7.036872737417e-05) (18,1.058045470413e-04) (19,6.333586451753e-05) (20,7.438816152327e-05) (21,8.027505392914e-05) (22,7.511981201686e-05)};
\addlegendentry{ARP T-CUR}
\addplot+[color=tSVD, mark=triangle*, dashed, line width=0.9pt] coordinates {(2,3.214702699390e-03) (3,3.659932368648e-04) (4,4.432359388782e-05) (5,5.415401130177e-06) (6,1.094210542000e-06) (7,8.851053867075e-07) (8,8.530930195787e-07) (9,8.234287046776e-07) (10,7.949866857896e-07) (11,7.674905684914e-07) (12,7.407595314475e-07) (13,7.147491762130e-07) (14,6.893904839251e-07) (15,6.646277000845e-07) (16,6.404154516039e-07) (17,6.167439678892e-07) (18,5.935909951193e-07) (19,5.709058025801e-07) (20,5.486649394852e-07) (21,5.269010313177e-07) (22,5.055202308874e-07)};
\addlegendentry{T-SVD}
\addplot+[color=tUniform, mark=diamond*, dash dot, line width=0.9pt] coordinates {(2,1.123035289941e-02) (3,3.950247700664e-03) (4,2.995682878390e-03) (5,2.222574600269e-03) (6,1.646409276687e-03) (7,1.324841713113e-03) (8,1.100180544362e-03) (9,9.227777862283e-04) (10,3.782900325277e-04) (11,9.163817228092e-04) (12,8.228722155877e-04) (13,5.654045518240e-04) (14,3.719659635267e-04) (15,3.097349728578e-04) (16,3.390730228116e-04) (17,2.712869408237e-04) (18,2.985453539617e-04) (19,1.974845164555e-04) (20,2.084913638897e-04) (21,1.787235583814e-04) (22,8.703754767728e-05)};
\addlegendentry{T Uniform Sampling}
\addplot+[color=tLeverage, mark=x, densely dotted, line width=0.9pt] coordinates {(2,1.354071682595e-02) (3,2.573476522273e-03) (4,6.744020373279e-04) (5,3.835273304851e-04) (6,1.719021347368e-04) (7,1.173219908079e-04) (8,2.683373519802e-04) (9,9.391280957784e-05) (10,9.158298644556e-05) (11,9.336257853117e-05) (12,9.572117345809e-05) (13,6.336187792270e-05) (14,8.735261732144e-05) (15,1.199372841232e-04) (16,5.412803120091e-05) (17,4.873118976962e-05) (18,4.985142256170e-05) (19,7.200964187535e-05) (20,7.145862821217e-05) (21,7.612684460123e-05) (22,3.832624597347e-05)};
\addlegendentry{T Leverage Scores Sampling}
\addplot+[color=tARP, mark=*, solid, line width=0.9pt] coordinates {(2,1.420602181621e-02) (3,9.634381967215e-04) (4,1.875429256314e-04) (5,5.678223345527e-05) (6,4.477195895442e-05) (7,4.320657431561e-05) (8,3.920299772227e-05) (9,3.930820208477e-05) (10,4.025234051095e-05) (11,3.933426413515e-05) (12,3.813214876939e-05) (13,3.839513720853e-05) (14,3.641814536762e-05) (15,3.632319251165e-05) (16,3.466146898711e-05) (17,3.470849982572e-05) (18,3.439270984444e-05) (19,3.361011928136e-05) (20,3.286512720910e-05) (21,3.284827501464e-05) (22,3.282310469944e-05)};
\addlegendentry{T-ARP}
\addplot+[color=tARPHouseholder, mark=none, densely dashed, line width=0.9pt] coordinates {(2,1.420602181621e-02) (3,9.634381967215e-04) (4,1.875429256314e-04) (5,5.678223345527e-05) (6,4.477195895442e-05) (7,4.320657431561e-05) (8,3.920299772227e-05) (9,3.930820208477e-05) (10,4.025234051095e-05) (11,3.933426413515e-05) (12,3.813214876939e-05) (13,3.839513720853e-05) (14,3.641814536762e-05) (15,3.632319251165e-05) (16,3.466146898711e-05) (17,3.470849982572e-05) (18,3.439270984444e-05) (19,3.361011928136e-05) (20,3.286512720910e-05) (21,3.284827501464e-05) (22,3.282310469944e-05)};
\addlegendentry{T-ARP (Householder)}
\end{axis}
\end{tikzpicture}


==> figures/random_tensor/relative_error_plot__old_.tex <==
\definecolor{arpTCUR}{RGB}{0,114,178}
\definecolor{tSVD}{RGB}{0,0,0}
\definecolor{tUniform}{RGB}{230,159,0}
\definecolor{tLeverage}{RGB}{0,158,115}
\definecolor{tARP}{RGB}{213,94,0}
\definecolor{tARPHouseholder}{RGB}{204,121,167}
\begin{tikzpicture}
\begin{axis}[%
width=\linewidth,
height=0.82\linewidth,
xlabel={Target rank / number of selected slices per mode \(r\)},
ylabel={Relative Error (log scale)},
ymode=log,
xtick={2,4,6,8,10,12,14,16,18,20,22},
grid=both,
legend style={font=\scriptsize, at={(0.5,-0.35)}, anchor=north, legend columns=2},
]
\addplot+[color=arpTCUR, mark=square*, solid, line width=0.9pt] coordinates {(2,1.498492461985e-02) (3,1.386281033930e-02) (4,1.240676291117e-02) (5,1.065963311109e-02) (6,8.186713667504e-03) (7,4.453351328486e-03) (8,1.797183778356e-03) (9,5.029879932812e-04) (10,5.457308777417e-05) (11,2.007515983149e-06) (12,1.813299732003e-06) (13,1.696441944522e-06) (14,1.576292117197e-06) (15,1.503760199170e-06) (16,1.442831102204e-06) (17,1.396335418799e-06) (18,1.356209594094e-06) (19,1.322252912832e-06) (20,1.293742087100e-06) (21,1.268855594067e-06) (22,1.249178493259e-06)};
\addlegendentry{ARP T-CUR}
\addplot+[color=tSVD, mark=triangle*, dashed, line width=0.9pt] coordinates {(2,1.189113042309e-02) (3,9.915439284091e-03) (4,7.993673666535e-03) (5,6.042669889783e-03) (6,3.917269562268e-03) (7,8.832094225527e-07) (8,8.519208035066e-07) (9,8.223175710976e-07) (10,7.938941725442e-07) (11,7.663890126856e-07) (12,7.396936335473e-07) (13,7.137155042947e-07) (14,6.884038909210e-07) (15,6.636855545418e-07) (16,6.395184113093e-07) (17,6.158846585594e-07) (18,5.927675980489e-07) (19,5.701137411343e-07) (20,5.478901532077e-07) (21,5.261435543331e-07) (22,5.048065465693e-07)};
\addlegendentry{T-SVD}
\addplot+[color=tUniform, mark=diamond*, dash dot, line width=0.9pt] coordinates {(2,1.535396752797e-02) (3,1.413012368617e-02) (4,1.257669398709e-02) (5,1.048494917897e-02) (6,7.556771107117e-03) (7,6.233610538167e-04) (8,2.260939992463e-04) (9,8.712668786946e-05) (10,3.032876939478e-05) (11,1.825374697945e-06) (12,1.662767729812e-06) (13,1.548971788254e-06) (14,1.460723927895e-06) (15,1.394532042512e-06) (16,1.335523058825e-06) (17,1.289051834047e-06) (18,1.252970712896e-06) (19,1.219439622880e-06) (20,1.189991186848e-06) (21,1.163624716624e-06) (22,1.140668883159e-06)};
\addlegendentry{T Uniform Sampling}
\addplot+[color=tLeverage, mark=x, densely dotted, line width=0.9pt] coordinates {(2,1.531280862220e-02) (3,1.413464679071e-02) (4,1.256399749960e-02) (5,1.045853167625e-02) (6,7.556912986447e-03) (7,7.002425393633e-04) (8,2.992801700026e-04) (9,1.080639679379e-04) (10,2.064309137046e-06) (11,3.522379419226e-05) (12,1.659681088533e-06) (13,1.547112941402e-06) (14,1.465178747436e-06) (15,1.393609818998e-06) (16,1.339558072262e-06) (17,1.290899007545e-06) (18,1.255021294524e-06) (19,1.216630631157e-06) (20,1.189311204639e-06) (21,1.163831625759e-06) (22,1.141205248160e-06)};
\addlegendentry{T Leverage Scores Sampling}
\addplot+[color=tARP, mark=*, solid, line width=0.9pt] coordinates {(2,1.514423488882e-02) (3,1.391355897639e-02) (4,1.228996214484e-02) (5,1.020574075255e-02) (6,7.339010562531e-03) (7,6.402755399901e-04) (8,2.417702037793e-04) (9,7.801803325509e-05) (10,1.932665689373e-06) (11,1.731059596773e-06) (12,1.615232822583e-06) (13,1.507824276786e-06) (14,1.432004408099e-06) (15,1.368340808043e-06) (16,1.316071693318e-06) (17,1.272930719167e-06) (18,1.238370258518e-06) (19,1.206930991312e-06) (20,1.179554721692e-06) (21,1.154801033085e-06) (22,1.135469373320e-06)};
\addlegendentry{T-ARP}
\addplot+[color=tARPHouseholder, mark=none, densely dashed, line width=0.9pt] coordinates {(2,1.514423488882e-02) (3,1.391355897639e-02) (4,1.228996214484e-02) (5,1.020574075255e-02) (6,7.339010562531e-03) (7,6.402755399901e-04) (8,2.417702037793e-04) (9,7.801803325509e-05) (10,1.932665689373e-06) (11,1.731059596773e-06) (12,1.615232822583e-06) (13,1.507824276786e-06) (14,1.432004408099e-06) (15,1.368340808043e-06) (16,1.316071693318e-06) (17,1.272930719167e-06) (18,1.238370258518e-06) (19,1.206930991312e-06) (20,1.179554721692e-06) (21,1.154801033085e-06) (22,1.135469373320e-06)};
\addlegendentry{T-ARP (Householder)}
\end{axis}
\end{tikzpicture}


==> tables/function_tensor/relative_error_table.tex <==
\begin{table}
\caption{RELATIVE\_ERROR values (mean ± std where multiple samples exist)}
\label{tab:func_tensor_relative_error}
\small
\begin{tabular}{lcccccc}
\toprule
\# Slices & ARP-T-CUR & T-SVD &  \makecell{T Uniform\\ Sampling} & \makecell{T Leverage\\ Scores Sampling} & T-ARP & \makecell{T-ARP\\(Householder)} \\
\midrule
2 & 0.023 & 0.003 & 0.007 & 0.007 & 0.014 & 0.014 \\
3 & 0.007 & 0.000 & 0.002 & 0.002 & 0.001 & 0.001 \\
4 & 0.006 & 0.000 & 0.001 & 0.001 & 0.000 & 0.000 \\
5 & 0.005 & 0.000 & 0.001 & 0.001 & 0.000 & 0.000 \\
6 & 0.004 & 0.000 & 0.001 & 0.001 & 0.000 & 0.000 \\
7 & 0.004 & 0.000 & 0.001 & 0.000 & 0.000 & 0.000 \\
8 & 0.004 & 0.000 & 0.001 & 0.000 & 0.000 & 0.000 \\
9 & 0.003 & 0.000 & 0.001 & 0.000 & 0.000 & 0.000 \\
10 & 0.003 & 0.000 & 0.001 & 0.000 & 0.000 & 0.000 \\
11 & 0.003 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
12 & 0.002 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
13 & 0.002 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
14 & 0.002 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
15 & 0.002 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
16 & 0.002 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
17 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
18 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
19 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
20 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
21 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
22 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/kodak/execution_time_table.tex <==
\begin{table}
\caption{EXECUTION_TIME values (mean ± std where multiple samples exist)}
\label{tab:kodak_execution_time}
\small
\begin{tabular}{lccccc}
\toprule
\# Slices & T-SVD & \makecell{T Uniform\\ Sampling} & \makecell{T Leverage\\ Scores Sampling} & T-ARP & \makecell{T-ARP\\(Householder)} \\
\midrule
10 & 0.577 $\pm$ 0.101 & 0.047 $\pm$ 0.105 & 0.070 $\pm$ 0.139 & 0.091 $\pm$ 0.179 & 0.090 $\pm$ 0.166 \\
20 & 0.515 $\pm$ 0.051 & 0.048 $\pm$ 0.079 & 0.081 $\pm$ 0.116 & 0.113 $\pm$ 0.106 & 0.127 $\pm$ 0.128 \\
40 & 0.528 $\pm$ 0.082 & 0.077 $\pm$ 0.110 & 0.135 $\pm$ 0.127 & 0.234 $\pm$ 0.118 & 0.252 $\pm$ 0.143 \\
60 & 0.553 $\pm$ 0.115 & 0.082 $\pm$ 0.076 & 0.161 $\pm$ 0.108 & 0.465 $\pm$ 0.063 & 0.507 $\pm$ 0.080 \\
80 & 0.532 $\pm$ 0.080 & 0.117 $\pm$ 0.072 & 0.211 $\pm$ 0.107 & 0.652 $\pm$ 0.099 & 0.739 $\pm$ 0.185 \\
100 & 0.558 $\pm$ 0.067 & 0.128 $\pm$ 0.088 & 0.249 $\pm$ 0.115 & 0.938 $\pm$ 0.103 & 0.739 $\pm$ 0.155 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/kodak/psnr_table_prev.tex <==
% \begin{table}[H]
% \centering
% \caption{Statistics of \emph{PSNR} measures on Kodak dataset ($\text{mean} \pm \text{std}$)}
% \label{tab:kodak_psnr}
% \footnotesize
% \begin{tabular}{|l|c|c|c|c|c|}
% %\toprule
% \# Slices & T-SVD & \makecell{T Uniform\\ Sampling} & \makecell{T Leverage\\ Scores Sampling} & T-ARP & \makecell{T-ARP\\(Householder)} \\\hline
% %\midrule
% 10 & 22.907 $\pm$ 2.585 & 18.528 $\pm$ 2.233 & 18.552 $\pm$ 2.210 & 18.759 $\pm$ 2.179 & 18.759 $\pm$ 2.179 \\\hline
% 20 & 24.825 $\pm$ 2.773 & 20.154 $\pm$ 2.320 & 20.207 $\pm$ 2.433 & 20.530 $\pm$ 2.468 & 20.530 $\pm$ 2.468 \\\hline
% 40 & 27.142 $\pm$ 3.013 & 21.851 $\pm$ 2.516 & 22.095 $\pm$ 2.620 & 22.551 $\pm$ 2.702 & 22.551 $\pm$ 2.702 \\\hline
% 60 & 28.830 $\pm$ 3.203 & 22.939 $\pm$ 2.585 & 23.435 $\pm$ 2.771 & 24.104 $\pm$ 2.932 & 24.101 $\pm$ 2.932 \\\hline
% 80 & 30.278 $\pm$ 3.360 & 24.116 $\pm$ 2.665 & 24.590 $\pm$ 2.881 & 25.272 $\pm$ 3.071 & 25.286 $\pm$ 3.071 \\\hline
% 100 & 31.605 $\pm$ 3.484 & 25.085 $\pm$ 2.754 & 25.546 $\pm$ 2.900 & 26.435 $\pm$ 3.273 & 26.442 $\pm$ 3.272 \\\hline
% %\bottomrule
% \end{tabular}
% \end{table}

\begin{table}[H]
\centering
\caption{Statistics of \emph{PSNR} measures on Kodak dataset ($\text{mean} \pm \text{std}$)}
\label{tab:kodak_psnr}
\footnotesize
\begin{tabular}{lcccccc}
\toprule
\# Slices & ARP T-CUR & T-SVD & \makecell{T Uniform\\ Sampling} & \makecell{T Leverage\\ Scores Sampling} & T-ARP & \makecell{T-ARP\\(Householder)} \\
\midrule
10 & 19.018 $\pm$ 2.243 & 22.907 $\pm$ 2.585 & 18.366 $\pm$ 2.057 & 18.710 $\pm$ 2.281 & 18.568 $\pm$ 2.090 & 18.568 $\pm$ 2.090 \\
20 & 20.842 $\pm$ 2.486 & 24.825 $\pm$ 2.773 & 20.118 $\pm$ 2.303 & 20.202 $\pm$ 2.291 & 20.680 $\pm$ 2.563 & 20.680 $\pm$ 2.563 \\
40 & 22.779 $\pm$ 2.704 & 27.142 $\pm$ 3.013 & 21.981 $\pm$ 2.462 & 22.080 $\pm$ 2.517 & 22.380 $\pm$ 2.701 & 22.380 $\pm$ 2.701 \\
60 & 24.064 $\pm$ 2.886 & 28.830 $\pm$ 3.203 & 23.063 $\pm$ 2.542 & 23.432 $\pm$ 2.692 & 23.895 $\pm$ 2.884 & 23.895 $\pm$ 2.884 \\
80 & 25.267 $\pm$ 3.074 & 30.278 $\pm$ 3.360 & 24.120 $\pm$ 2.671 & 24.521 $\pm$ 2.789 & 24.989 $\pm$ 2.949 & 24.989 $\pm$ 2.949 \\
100 & 26.190 $\pm$ 3.139 & 31.605 $\pm$ 3.484 & 25.045 $\pm$ 2.782 & 25.506 $\pm$ 2.918 & 25.932 $\pm$ 3.025 & 25.932 $\pm$ 3.025 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/kodak/relative_error_table_prev.tex <==
% \begin{table}[H]
% \centering
% \caption{Statistics of \emph{relative error} measures on Kodak dataset ($\text{mean} \pm \text{std}$)}
% \label{tab:kodak_relative_error}
% \footnotesize
% \begin{tabular}{|l|c|c|c|c|c|}
% %\toprule
% \# Slices & T-SVD & \makecell{T Uniform\\ Sampling} & \makecell{T Leverage\\ Scores Sampling} & T-ARP & \makecell{T-ARP\\(Householder)} \\\hline
% %\midrule
% 10 & 0.171 $\pm$ 0.070 & 0.286 $\pm$ 0.103 & 0.286 $\pm$ 0.104 & 0.276 $\pm$ 0.096 & 0.276 $\pm$ 0.096 \\\hline
% 20 & 0.137 $\pm$ 0.060 & 0.235 $\pm$ 0.089 & 0.235 $\pm$ 0.091 & 0.226 $\pm$ 0.087 & 0.226 $\pm$ 0.087 \\\hline
% 40 & 0.106 $\pm$ 0.049 & 0.192 $\pm$ 0.076 & 0.189 $\pm$ 0.078 & 0.179 $\pm$ 0.076 & 0.179 $\pm$ 0.076 \\\hline
% 60 & 0.088 $\pm$ 0.042 & 0.170 $\pm$ 0.069 & 0.162 $\pm$ 0.070 & 0.151 $\pm$ 0.068 & 0.151 $\pm$ 0.068 \\\hline
% 80 & 0.075 $\pm$ 0.037 & 0.148 $\pm$ 0.063 & 0.142 $\pm$ 0.064 & 0.132 $\pm$ 0.061 & 0.132 $\pm$ 0.061 \\\hline
% 100 & 0.064 $\pm$ 0.033 & 0.133 $\pm$ 0.058 & 0.127 $\pm$ 0.058 & 0.117 $\pm$ 0.056 & 0.116 $\pm$ 0.056 \\\hline
% %\bottomrule
% \end{tabular}
% \end{table}

\begin{table}[H]
\centering
\caption{Statistics of \emph{relative error} measures on Kodak dataset ($\text{mean} \pm \text{std}$)}
\label{tab:kodak_relative_error}
\footnotesize
\begin{tabular}{lcccccc}
\toprule
\# Slices & ARP T-CUR & T-SVD & \makecell{T Uniform\\ Sampling} & \makecell{T Leverage\\ Scores Sampling} & T-ARP & \makecell{T-ARP\\(Householder)} \\
\midrule
10 & 0.257 $\pm$ 0.084 & 0.167 $\pm$ 0.065 & 0.274 $\pm$ 0.081 & 0.267 $\pm$ 0.081 & 0.269 $\pm$ 0.083 & 0.269 $\pm$ 0.083 \\
20 & 0.211 $\pm$ 0.079 & 0.135 $\pm$ 0.057 & 0.227 $\pm$ 0.079 & 0.225 $\pm$ 0.076 & 0.215 $\pm$ 0.081 & 0.215 $\pm$ 0.081 \\
40 & 0.170 $\pm$ 0.070 & 0.105 $\pm$ 0.048 & 0.185 $\pm$ 0.070 & 0.186 $\pm$ 0.068 & 0.178 $\pm$ 0.071 & 0.178 $\pm$ 0.071 \\
60 & 0.149 $\pm$ 0.065 & 0.087 $\pm$ 0.041 & 0.164 $\pm$ 0.064 & 0.163 $\pm$ 0.063 & 0.151 $\pm$ 0.064 & 0.151 $\pm$ 0.064 \\
80 & 0.130 $\pm$ 0.059 & 0.074 $\pm$ 0.037 & 0.146 $\pm$ 0.060 & 0.145 $\pm$ 0.057 & 0.134 $\pm$ 0.059 & 0.134 $\pm$ 0.059 \\
100 & 0.118 $\pm$ 0.055 & 0.064 $\pm$ 0.032 & 0.132 $\pm$ 0.056 & 0.131 $\pm$ 0.053 & 0.120 $\pm$ 0.054 & 0.120 $\pm$ 0.054 \\
\bottomrule
\end{tabular}
\end{table}

==> tables/kodak/ssim_table_prev.tex <==
\begin{table}[H]
\centering
\caption{Statistics of \emph{SSIM} measures on Kodak dataset ($\text{mean} \pm \text{std}$)}
\label{tab:kodak_ssim}
\footnotesize
\begin{tabular}{lcccccc}
\toprule
\# Slices & ARP T-CUR & T-SVD & \makecell{T Uniform\\ Sampling} & \makecell{T Leverage\\ Scores Sampling} & T-ARP & \makecell{T-ARP\\(Householder)} \\
\midrule
10 & 0.428 $\pm$ 0.130 & 0.589 $\pm$ 0.128 & 0.426 $\pm$ 0.135 & 0.431 $\pm$ 0.134 & 0.423 $\pm$ 0.130 & 0.423 $\pm$ 0.130 \\
20 & 0.471 $\pm$ 0.130 & 0.643 $\pm$ 0.113 & 0.465 $\pm$ 0.128 & 0.466 $\pm$ 0.126 & 0.471 $\pm$ 0.132 & 0.471 $\pm$ 0.132 \\
40 & 0.536 $\pm$ 0.123 & 0.718 $\pm$ 0.094 & 0.522 $\pm$ 0.120 & 0.519 $\pm$ 0.121 & 0.523 $\pm$ 0.124 & 0.523 $\pm$ 0.124 \\
60 & 0.586 $\pm$ 0.117 & 0.771 $\pm$ 0.080 & 0.563 $\pm$ 0.113 & 0.564 $\pm$ 0.114 & 0.583 $\pm$ 0.118 & 0.583 $\pm$ 0.118 \\
80 & 0.631 $\pm$ 0.110 & 0.812 $\pm$ 0.070 & 0.605 $\pm$ 0.106 & 0.603 $\pm$ 0.104 & 0.628 $\pm$ 0.110 & 0.628 $\pm$ 0.110 \\
100 & 0.670 $\pm$ 0.101 & 0.844 $\pm$ 0.060 & 0.643 $\pm$ 0.099 & 0.641 $\pm$ 0.096 & 0.668 $\pm$ 0.102 & 0.668 $\pm$ 0.102 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/random_tensor/relative_error_table.tex <==
\begin{table}
\caption{RELATIVE\_ERROR values (mean ± std where multiple samples exist)}
\label{tab:rand_tensor_relative_error}
\small
\begin{tabular}{lcccccc}
\toprule
\# Slices & ARP-T-CUR & T-SVD &  \makecell{T Uniform\\ Sampling} & \makecell{T Leverage\\ Scores Sampling} & T-ARP & \makecell{T-ARP\\(Householder)} \\
\midrule
2 & 0.015 & 0.012 & 0.015 & 0.015 & 0.015 & 0.015 \\
3 & 0.014 & 0.010 & 0.014 & 0.014 & 0.014 & 0.014 \\
4 & 0.012 & 0.008 & 0.013 & 0.013 & 0.012 & 0.012 \\
5 & 0.010 & 0.006 & 0.011 & 0.011 & 0.010 & 0.010 \\
6 & 0.007 & 0.004 & 0.008 & 0.008 & 0.007 & 0.007 \\
7 & 0.001 & 0.000 & 0.001 & 0.001 & 0.000 & 0.000 \\
8 & 0.001 & 0.000 & 0.000 & 0.000 & 0.001 & 0.001 \\
9 & 0.001 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
10 & 0.001 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
11 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
12 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
13 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
14 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
15 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
16 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
17 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
18 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
19 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
20 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
21 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
22 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\bottomrule
\end{tabular}
\end{table}

